Gravitational bremsstrahlung from Yukawa and nucleon collisions

We obtain the gravitational emission from particles scattering via the Yukawa interaction, presenting both classical and approximate quantum results. We also estimate the contribution from the tensor part of the internucleon interaction. This emission is the main source of a very-high frequency component to the stochastic background in the Solar System and in neutron stars. The emission from the Sun (allowing for Debye screening) and from a typical neutron star are obtained. The gravitational wave luminosity of the Sun is $41 \pm 10$ MW.

==> Sigmafig.tex <==
\begin{loglogaxis}[
xmin= 0.001, xmax= 1000,
xlabel={$\Omega$},
ylabel={$\chi \Omega^{3/2}$},
ylabel near ticks,
]
\addplot [dotted,blue]
coordinates {
( 0.001, 6.71092823e-7)
( 0.001149757, 8.95917486e-7)
( 0.00132194115, 1.19560018e-6)
( 0.00151991108, 1.59491926e-6)
( 0.0017475284, 2.12680895e-6)
( 0.002009233, 2.83502963e-6)
( 0.0023101297, 3.77770763e-6)
( 0.00265608778, 5.03202654e-6)
( 0.00305385551, 6.70044202e-6)
( 0.00351119173, 8.91891225e-6)
( 0.00403701726, 1.18677934e-5)
( 0.00464158883, 1.57862574e-5)
( 0.00533669923, 2.09913621e-5)
( 0.00613590727, 2.79032633e-5)
( 0.00705480231, 3.70785305e-5)
( 0.00811130831, 4.92541454e-5)
( 0.00932603347, 6.54055741e-5)
( 0.0107226722, 8.68233651e-5)
( 0.0123284674, 0.000115214107)
( 0.0141747416, 0.000152833391)
( 0.0162975083, 0.000202660766)
( 0.0187381742, 0.000268629732)
( 0.0215443469, 0.000355929782)
( 0.0247707636, 0.000471402578)
( 0.0284803587, 0.000624060997)
( 0.0327454916, 0.000825768211)
( 0.0376493581, 0.00109212485)
( 0.0432876128, 0.00144362617)
( 0.0497702356, 0.00190716891)
( 0.0572236766, 0.00251800975)
( 0.0657933225, 0.00332230605)
( 0.0756463328, 0.00438040472)
( 0.0869749003, 0.00577109054)
( 0.1, 0.00759706065)
( 0.1149757, 0.00999196197)
( 0.132194115, 0.0131294144)
( 0.151991108, 0.0172345489)
( 0.17475284, 0.022598721)
( 0.2009233, 0.0295982185)
( 0.23101297, 0.0387179809)
( 0.265608778, 0.0505815809)
( 0.305385551, 0.065989012)
( 0.351119173, 0.0859641719)
( 0.403701726, 0.11181436)
( 0.464158883, 0.145204618)
( 0.533669923, 0.188250376)
( 0.613590727, 0.243632619)
( 0.705480231, 0.314740738)
( 0.811130831, 0.405849356)
( 0.932603347, 0.52233685)
( 1.07226722, 0.670955004)
( 1.23284674, 0.860161422)
( 1.41747416, 1.10052896)
( 1.62975083, 1.40524976)
( 1.87381742, 1.79075564)
( 2.15443469, 2.2774816)
( 2.47707636, 2.89080553)
( 2.84803587, 3.66220512)
( 3.27454916, 4.63068252)
( 3.76493581, 5.84451906)
( 4.32876128, 7.36343741)
( 4.97702356, 9.26126602)
( 5.72236766, 11.6292235)
( 6.57933225, 14.5799676)
( 7.56463328, 18.2525873)
( 8.69749003, 22.8187578)
( 10, 28.4903308)
( 11.49757, 35.5286926)
( 13.2194115, 44.2563043)
( 15.1991108, 55.0709301)
( 17.475284, 68.4631824)
( 20.09233, 85.0381534)
( 23.101297, 105.542087)
( 26.5608778, 130.895266)
( 30.5385551, 162.232552)
( 35.1119173, 200.953378)
( 40.3701726, 248.78338)
( 46.4158883, 307.850377)
( 53.3669923, 380.778052)
( 61.3590727, 470.801452)
( 70.5480231, 581.90937)
( 81.1130831, 719.019901)
( 93.2603347, 888.19687)
( 107.226722, 1096.91665)
( 123.284674, 1354.39714)
( 141.747416, 1672.0033)
( 162.975083, 2063.74715)
( 187.381742, 2546.90421)
( 215.443469, 3142.77345)
( 247.707636, 3877.6142)
( 284.803587, 4783.80124)
( 327.454916, 5901.24881)
( 376.493581, 7279.16629)
( 432.876128, 8978.22258)
( 497.702356, 11073.2145)
( 572.236766, 13656.3567)
( 657.933225, 16841.3372)
( 756.463328, 20768.3175)
( 869.749003, 25610.0974)
( 1000, 31579.7143)
};
\addplot [dashed,red]
coordinates {
( 0.001, 3.08457339e-11)
( 0.001149757, 4.68709536e-11)
( 0.00132194115, 7.12190285e-11)
( 0.00151991108, 1.08210506e-10)
( 0.0017475284, 1.64407341e-10)
( 0.002009233, 2.49774496e-10)
( 0.0023101297, 3.79442888e-10)
( 0.00265608778, 5.76384051e-10)
( 0.00305385551, 8.75466997e-10)
( 0.00351119173, 1.32961015e-9)
( 0.00403701726, 2.01910614e-9)
( 0.00464158883, 3.06575116e-9)
( 0.00533669923, 4.65424388e-9)
( 0.00613590727, 7.06457735e-9)
( 0.00705480231, 1.07210413e-8)
( 0.00811130831, 1.62663016e-8)
( 0.00932603347, 2.46732999e-8)
( 0.0107226722, 3.74141308e-8)
( 0.0123284674, 5.67146393e-8)
( 0.0141747416, 8.59377955e-8)
( 0.0162975083, 1.30160195e-7)
( 0.0187381742, 1.97037625e-7)
( 0.0215443469, 2.98102333e-7)
( 0.0247707636, 4.5070338e-7)
( 0.0284803587, 6.80902204e-7)
( 0.0327454916, 1.02778234e-6)
( 0.0376493581, 1.54984494e-6)
( 0.0432876128, 2.33446783e-6)
( 0.0497702356, 3.5118425e-6)
( 0.0572236766, 5.27542148e-6)
( 0.0657933225, 7.91177367e-6)
( 0.0756463328, 1.18439429e-5)
( 0.0869749003, 1.7694041e-5)
( 0.1, 2.63730098e-5)
( 0.1149757, 3.92084031e-5)
( 0.132194115, 5.81248315e-5)
( 0.151991108, 8.58965419e-5)
( 0.17475284, 0.000126497615)
( 0.2009233, 0.00018558256)
( 0.23101297, 0.000271138719)
( 0.265608778, 0.000394361792)
( 0.305385551, 0.000570816865)
( 0.351119173, 0.000821959325)
( 0.403701726, 0.00117710274)
( 0.464158883, 0.00167593409)
( 0.533669923, 0.00237169051)
( 0.613590727, 0.0033351265)
( 0.705480231, 0.00465941667)
( 0.811130831, 0.00646615801)
( 0.932603347, 0.00891265866)
( 1.07226722, 0.0122007284)
( 1.23284674, 0.0165872226)
( 1.41747416, 0.0223966354)
( 1.62975083, 0.030036096)
( 1.87381742, 0.0400131851)
( 2.15443469, 0.0529570758)
( 2.47707636, 0.0696435937)
( 2.84803587, 0.0910249055)
( 3.27454916, 0.118264677)
( 3.76493581, 0.152779694)
( 4.32876128, 0.196289111)
( 4.97702356, 0.250872706)
( 5.72236766, 0.319039761)
( 6.57933225, 0.403810454)
( 7.56463328, 0.508811986)
( 8.69749003, 0.638392054)
( 10, 0.797752707)
( 11.49757, 0.99310817)
( 13.2194115, 1.2318708)
( 15.1991108, 1.52287007)
( 17.475284, 1.87661035)
( 20.09233, 2.30557406)
( 23.101297, 2.82457823)
( 26.5608778, 3.4511934)
( 30.5385551, 4.20623574)
( 35.1119173, 5.11434481)
( 40.3701726, 6.20466167)
( 46.4158883, 7.51162426)
( 53.3669923, 9.07590017)
( 61.3590727, 10.94548)
( 70.5480231, 13.1769585)
( 81.1130831, 15.8370351)
( 93.2603347, 19.0042713)
( 107.226722, 22.7711471)
( 123.284674, 27.2464682)
( 141.747416, 32.5581814)
( 162.975083, 38.8566675)
( 187.381742, 46.318591)
( 215.443469, 55.1513996)
( 247.707636, 65.5985823)
( 284.803587, 77.9458116)
( 327.454916, 92.5281174)
( 376.493581, 109.738263)
( 432.876128, 130.036525)
( 497.702356, 153.962102)
( 572.236766, 182.146435)
( 657.933225, 215.328739)
( 756.463328, 254.374121)
( 869.749003, 300.294713)
( 1000, 354.2743)
};
\addplot [thick,black]
coordinates {
( 0.001, 3.77262124e-10)
( 0.001149757, 5.57512753e-10)
( 0.00132194115, 8.23050556e-10)
( 0.00151991108, 1.21381384e-9)
( 0.0017475284, 1.7882366e-9)
( 0.002009233, 2.63171178e-9)
( 0.0023101297, 3.86887634e-9)
( 0.00265608778, 5.6814194e-9)
( 0.00305385551, 8.3338586e-9)
( 0.00351119173, 1.22107945e-8)
( 0.00403701726, 1.78706707e-8)
( 0.00464158883, 2.61232282e-8)
( 0.00533669923, 3.81409086e-8)
( 0.00613590727, 5.56188143e-8)
( 0.00705480231, 8.1003965e-8)
( 0.00811130831, 1.17823257e-7)
( 0.00932603347, 1.71151685e-7)
( 0.0107226722, 2.4827944e-7)
( 0.0123284674, 3.59660268e-7)
( 0.0141747416, 5.20256615e-7)
( 0.0162975083, 7.51442975e-7)
( 0.0187381742, 1.08369226e-6)
( 0.0215443469, 1.56035724e-6)
( 0.0247707636, 2.24297846e-6)
( 0.0284803587, 3.21871283e-6)
( 0.0327454916, 4.61069769e-6)
( 0.0376493581, 6.59246271e-6)
( 0.0432876128, 9.40790116e-6)
( 0.0497702356, 1.3398844e-5)
( 0.0572236766, 1.90429848e-5)
( 0.0657933225, 2.70058305e-5)
( 0.0756463328, 3.8211563e-5)
( 0.0869749003, 5.39392664e-5)
( 0.1, 7.59529923e-5)
( 0.1149757, 0.000106676707)
( 0.132194115, 0.000149428422)
( 0.151991108, 0.000208731875)
( 0.17475284, 0.000290729209)
( 0.2009233, 0.000403724287)
( 0.23101297, 0.000558893902)
( 0.265608778, 0.00077121326)
( 0.305385551, 0.00106065308)
( 0.351119173, 0.00145371866)
( 0.403701726, 0.00198541648)
( 0.464158883, 0.00270175193)
( 0.533669923, 0.00366288244)
( 0.613590727, 0.00494707453)
( 0.705480231, 0.00665564106)
( 0.811130831, 0.00891906764)
( 0.932603347, 0.0119045739)
( 1.07226722, 0.0158253996)
( 1.23284674, 0.0209521542)
( 1.41747416, 0.027626629)
( 1.62975083, 0.0362785368)
( 1.87381742, 0.0474457224)
( 2.15443469, 0.0617984797)
( 2.47707636, 0.0801687133)
( 2.84803587, 0.103584803)
( 3.27454916, 0.133313166)
( 3.76493581, 0.170907664)
( 4.32876128, 0.218268191)
( 4.97702356, 0.277709945)
( 5.72236766, 0.352045163)
( 6.57933225, 0.444679295)
( 7.56463328, 0.559723934)
( 8.69749003, 0.702129105)
( 10, 0.87783793)
( 11.49757, 1.09396707)
( 13.2194115, 1.35901688)
( 15.1991108, 1.68311571)
( 17.475284, 2.07830359)
( 20.09233, 2.55886098)
( 23.101297, 3.14168947)
( 26.5608778, 3.84675219)
( 30.5385551, 4.69758259)
( 35.1119173, 5.72187206)
( 40.3701726, 6.95214795)
( 46.4158883, 8.42655561)
( 53.3669923, 10.1897599)
( 61.3590727, 12.2939844)
( 70.5480231, 14.8002084)
( 81.1130831, 17.7795457)
( 93.2603347, 21.3148336)
( 107.226722, 25.5024613)
( 123.284674, 30.4544766)
( 141.747416, 36.3010108)
( 162.975083, 43.1930711)
( 187.381742, 51.3057552)
( 215.443469, 60.8419523)
( 247.707636, 72.0366038)
( 284.803587, 85.1616073)
( 327.454916, 100.531463)
( 376.493581, 118.509771)
( 432.876128, 139.516711)
( 497.702356, 164.037654)
( 572.236766, 192.633064)
( 657.933225, 225.949907)
( 756.463328, 264.734765)
( 869.749003, 309.848944)
( 1000, 362.285838)
};
\addplot [thin,black]
coordinates {
( 0.001, 7.18548059e-6)
( 0.001149757, 8.25982456e-6)
( 0.00132194115, 9.51088218e-6)
( 0.00151991108, 1.09703982e-5)
( 0.0017475284, 1.26762482e-5)
( 0.002009233, 1.46736889e-5)
( 0.0023101297, 1.70168754e-5)
( 0.00265608778, 1.97707008e-5)
( 0.00305385551, 2.30130316e-5)
( 0.00351119173, 2.68374236e-5)
( 0.00403701726, 3.13564269e-5)
( 0.00464158883, 3.67056082e-5)
( 0.00533669923, 4.30484506e-5)
( 0.00613590727, 5.0582327e-5)
( 0.00705480231, 5.95457856e-5)
( 0.00811130831, 7.0227442e-5)
( 0.00932603347, 8.29768369e-5)
( 0.0107226722, 9.82177035e-5)
( 0.0123284674, 0.000116464183)
( 0.0141747416, 0.000138340658)
( 0.0162975083, 0.000164606014)
( 0.0187381742, 0.000196183337)
( 0.0215443469, 0.000234196274)
( 0.0247707636, 0.000280013558)
( 0.0284803587, 0.000335303568)
( 0.0327454916, 0.000402101176)
( 0.0376493581, 0.000482889683)
( 0.0432876128, 0.000580701262)
( 0.0497702356, 0.00069924011)
( 0.0572236766, 0.000843033446)
( 0.0657933225, 0.00101761668)
( 0.0756463328, 0.00122976048)
( 0.0869749003, 0.0014877492)
( 0.1, 0.00180172229)
( 0.1149757, 0.00218409282)
( 0.132194115, 0.0026500605)
( 0.151991108, 0.00321824039)
( 0.17475284, 0.00391143297)
( 0.2009233, 0.0047575673)
( 0.23101297, 0.00579085527)
( 0.265608778, 0.00705320367)
( 0.305385551, 0.0085959405)
( 0.351119173, 0.0104819238)
( 0.403701726, 0.0127881156)
( 0.464158883, 0.0156087208)
( 0.533669923, 0.0190590107)
( 0.613590727, 0.0232799752)
( 0.705480231, 0.028443975)
( 0.811130831, 0.0347616016)
( 0.932603347, 0.0424899859)
( 1.07226722, 0.0519428495)
( 1.23284674, 0.063502638)
( 1.41747416, 0.0776351427)
( 1.62975083, 0.0949070835)
( 1.87381742, 0.116007209)
( 2.15443469, 0.141771559)
( 2.47707636, 0.173213649)
( 2.84803587, 0.211560434)
( 3.27454916, 0.258295081)
( 3.76493581, 0.315207692)
( 4.32876128, 0.384455321)
( 4.97702356, 0.468632828)
( 5.72236766, 0.570856304)
( 6.57933225, 0.6948611)
( 7.56463328, 0.845116736)
( 8.69749003, 1.02696134)
( 10, 1.24675859)
( 11.49757, 1.51208055)
( 13.2194115, 1.83192055)
( 15.1991108, 2.21694015)
( 17.475284, 2.67975576)
( 20.09233, 3.2352706)
( 23.101297, 3.90105873)
( 26.5608778, 4.69780898)
( 30.5385551, 5.6498376)
( 35.1119173, 6.78567998)
( 40.3701726, 8.13877309)
( 46.4158883, 9.74824227)
( 53.3669923, 11.659808)
( 61.3590727, 13.9268105)
( 70.5480231, 16.6115124)
( 81.1130831, 19.7862857)
( 93.2603347, 23.5354059)
( 107.226722, 27.9567894)
( 123.284674, 33.1641281)
( 141.747416, 39.289324)
( 162.975083, 46.4852913)
( 187.381742, 54.9291819)
( 215.443469, 64.8260983)
( 247.707636, 76.4133668)
( 284.803587, 89.9654563)
( 327.454916, 105.799638)
( 376.493581, 124.282502)
( 432.876128, 145.837452)
( 497.702356, 170.953334)
( 572.236766, 200.194368)
( 657.933225, 234.211566)
( 756.463328, 273.755882)
( 869.749003, 319.693336)
( 1000, 373.022414)
};
\end{loglogaxis}


==> chi0fig.tex <==
\begin{loglogaxis}[
xmin= 0.0001, xmax= 100,
xlabel={$\Omega$},
ylabel={$\chi$},
ylabel near ticks,
grid=both
]
\addplot []
coordinates {
( 1e-6, 0.000247549689)
( 1.20450354e-6, 0.000282515209)
( 1.45082878e-6, 0.00032223085)
( 1.7475284e-6, 0.000367311305)
( 2.10490414e-6, 0.000418445989)
( 2.53536449e-6, 0.000476407387)
( 3.05385551e-6, 0.00054206026)
( 3.67837977e-6, 0.000616371706)
( 4.43062146e-6, 0.000700422231)
( 5.33669923e-6, 0.000795417857)
( 6.42807312e-6, 0.000902703525)
( 7.74263683e-6, 0.00102377694)
( 9.32603347e-6, 0.00116030528)
( 1.12332403e-5, 0.00131414181)
( 1.35304777e-5, 0.00148734473)
( 1.62975083e-5, 0.0016821976)
( 1.96304065e-5, 0.00190123145)
( 2.36448941e-5, 0.00214724885)
( 2.84803587e-5, 0.00242334998)
( 3.43046929e-5, 0.00273296097)
( 4.1320124e-5, 0.00307986465)
( 4.97702356e-5, 0.0034682336)
( 5.9948425e-5, 0.00390266654)
( 7.22080902e-5, 0.00438822732)
( 8.69749003e-5, 0.00493048733)
( 0.000104761575, 0.00553557165)
( 0.000126185688, 0.00621020908)
( 0.000151991108, 0.00696178652)
( 0.000183073828, 0.00779840821)
( 0.000220513074, 0.00872896019)
( 0.000265608778, 0.0097631806)
( 0.000319926714, 0.0109117363)
( 0.000385352859, 0.0121863068)
( 0.000464158883, 0.0135996755)
( 0.000559081018, 0.0151658295)
( 0.000673415066, 0.0169000688)
( 0.000811130831, 0.018819125)
( 0.000977009957, 0.0209412904)
( 0.00117681195, 0.0232865582)
( 0.00141747416, 0.0258767733)
( 0.00170735265, 0.0287357952)
( 0.00205651231, 0.0318896701)
( 0.00247707636, 0.0353668131)
( 0.00298364724, 0.0391981977)
( 0.00359381366, 0.043417549)
( 0.00432876128, 0.0480615371)
( 0.00521400829, 0.0531699637)
( 0.00628029144, 0.0587859338)
( 0.00756463328, 0.0649560021)
( 0.00911162756, 0.07173028)
( 0.0109749877, 0.0791624862)
( 0.0132194115, 0.0873099215)
( 0.0159228279, 0.0962333409)
( 0.0191791026, 0.105996698)
( 0.023101297, 0.116666725)
( 0.027825594, 0.128312321)
( 0.0335160265, 0.141003699)
( 0.0403701726, 0.154811262)
( 0.0486260158, 0.169804175)
( 0.0585702082, 0.186048591)
( 0.0705480231, 0.203605515)
( 0.0849753436, 0.222528296)
( 0.102353102, 0.24285977)
( 0.123284674, 0.264629077)
( 0.148496826, 0.28784824)
( 0.178864953, 0.312508626)
( 0.215443469, 0.33857743)
( 0.259502421, 0.365994423)
( 0.312571585, 0.394669192)
( 0.376493581, 0.42447917)
( 0.453487851, 0.455268766)
( 0.546227722, 0.486849882)
( 0.657933225, 0.519004072)
( 0.792482898, 0.5514865)
( 0.954548457, 0.584031719)
( 1.149757, 0.616361162)
( 1.38488637, 0.64819199)
( 1.66810054, 0.679246811)
( 2.009233, 0.70926362)
( 2.42012826, 0.738005207)
( 2.91505306, 0.765267322)
( 3.51119173, 0.790884956)
( 4.22924287, 0.8147363)
( 5.09413801, 0.836744189)
( 6.13590727, 0.856875095)
( 7.39072203, 0.875135967)
( 8.90215085, 0.891569397)
( 10.7226722, 0.906247661)
( 12.9154967, 0.91926623)
( 15.5567614, 0.93073726)
( 18.7381742, 0.940783471)
( 22.5701972, 0.94953273)
( 27.1858824, 0.957113485)
( 32.7454916, 0.963651135)
( 39.4420606, 0.9692653)
( 47.5081016, 0.97406793)
( 57.2236766, 0.97816212)
( 68.926121, 0.981641523)
( 83.0217568, 0.984590221)
( 100, 0.987082948)
};
\end{loglogaxis}


==> chisfig.tex <==
\begin{loglogaxis}[
xmin= 0.001, xmax= 1000,
xlabel={$\Omega$},
ylabel={$\chi$},
ylabel near ticks,
]
\addplot [dotted,blue]
coordinates {
( 0.001, 0.0212218184)
( 0.001149757, 0.0229804708)
( 0.00132194115, 0.0248752692)
( 0.00151991108, 0.0269160564)
( 0.0017475284, 0.0291133456)
( 0.002009233, 0.0314783636)
( 0.0023101297, 0.0340230935)
( 0.00265608778, 0.0367603203)
( 0.00305385551, 0.0397036768)
( 0.00351119173, 0.0428676892)
( 0.00403701726, 0.0462678234)
( 0.00464158883, 0.0499205293)
( 0.00533669923, 0.0538432827)
( 0.00613590727, 0.0580546239)
( 0.00705480231, 0.0625741907)
( 0.00811130831, 0.0674227441)
( 0.00932603347, 0.0726221843)
( 0.0107226722, 0.0781955554)
( 0.0123284674, 0.0841670339)
( 0.0141747416, 0.0905618994)
( 0.0162975083, 0.0974064825)
( 0.0187381742, 0.104728087)
( 0.0215443469, 0.11255488)
( 0.0247707636, 0.120915747)
( 0.0284803587, 0.129840105)
( 0.0327454916, 0.139357673)
( 0.0376493581, 0.149498186)
( 0.0432876128, 0.160291057)
( 0.0497702356, 0.171764976)
( 0.0572236766, 0.18394745)
( 0.0657933225, 0.196864274)
( 0.0756463328, 0.210538934)
( 0.0869749003, 0.224991949)
( 0.1, 0.240240152)
( 0.1149757, 0.256295914)
( 0.132194115, 0.273166334)
( 0.151991108, 0.290852398)
( 0.17475284, 0.309348131)
( 0.2009233, 0.328639769)
( 0.23101297, 0.348704984)
( 0.265608778, 0.369512184)
( 0.305385551, 0.391019935)
( 0.351119173, 0.413176551)
( 0.403701726, 0.435919877)
( 0.464158883, 0.459177319)
( 0.533669923, 0.482866149)
( 0.613590727, 0.506894117)
( 0.705480231, 0.531160395)
( 0.811130831, 0.555556839)
( 0.932603347, 0.579969575)
( 1.07226722, 0.604280877)
( 1.23284674, 0.628371276)
( 1.41747416, 0.652121842)
( 1.62975083, 0.675416554)
( 1.87381742, 0.698144658)
( 2.15443469, 0.720202919)
( 2.47707636, 0.741497662)
( 2.84803587, 0.76194651)
( 3.27454916, 0.781479759)
( 3.76493581, 0.800041316)
( 4.32876128, 0.817589198)
( 4.97702356, 0.834095568)
( 5.72236766, 0.849546357)
( 6.57933225, 0.863940498)
( 7.56463328, 0.877288861)
( 8.69749003, 0.889612936)
( 10, 0.900943366)
( 11.49757, 0.911318394)
( 13.2194115, 0.920782301)
( 15.1991108, 0.929383888)
( 17.475284, 0.937175052)
( 20.09233, 0.944209502)
( 23.101297, 0.950541613)
( 26.5608778, 0.956225461)
( 30.5385551, 0.961314011)
( 35.1119173, 0.965858472)
( 40.3701726, 0.969907807)
( 46.4158883, 0.973508369)
( 53.3669923, 0.976703665)
( 61.3590727, 0.979534217)
( 70.5480231, 0.982037512)
( 81.1130831, 0.984248015)
( 93.2603347, 0.986197243)
( 107.226722, 0.987913874)
( 123.284674, 0.98942389)
( 141.747416, 0.990750732)
( 162.975083, 0.991915479)
( 187.381742, 0.992937017)
( 215.443469, 0.993832227)
( 247.707636, 0.994616149)
( 284.803587, 0.995302156)
( 327.454916, 0.995902111)
( 376.493581, 0.996426518)
( 432.876128, 0.99688466)
( 497.702356, 0.997284728)
( 572.236766, 0.997633941)
( 657.933225, 0.99793865)
( 756.463328, 0.998204438)
( 869.749003, 0.998436206)
( 1000, 0.998638251)
};
\addplot [dashed,red]
coordinates {
( 0.001, 9.75427753e-7)
( 0.001149757, 1.20224976e-6)
( 0.00132194115, 1.48175999e-6)
( 0.00151991108, 1.82617399e-6)
( 0.0017475284, 2.25053019e-6)
( 0.002009233, 2.77333694e-6)
( 0.0023101297, 3.41736897e-6)
( 0.00265608778, 4.21064201e-6)
( 0.00305385551, 5.18760681e-6)
( 0.00351119173, 6.39061276e-6)
( 0.00403701726, 7.87169469e-6)
( 0.00464158883, 9.69475642e-6)
( 0.00533669923, 1.19382329e-5)
( 0.00613590727, 1.46983303e-5)
( 0.00705480231, 1.80929631e-5)
( 0.00811130831, 2.22665256e-5)
( 0.00932603347, 2.7395661e-5)
( 0.0107226722, 3.36962146e-5)
( 0.0123284674, 4.1431584e-5)
( 0.0141747416, 5.09227069e-5)
( 0.0162975083, 6.25599471e-5)
( 0.0187381742, 7.68171616e-5)
( 0.0215443469, 9.42682349e-5)
( 0.0247707636, 0.000115606359)
( 0.0284803587, 0.000141666302)
( 0.0327454916, 0.000173449829)
( 0.0376493581, 0.000212154323)
( 0.0432876128, 0.000259204442)
( 0.0497702356, 0.000316286376)
( 0.0572236766, 0.000385383864)
( 0.0657933225, 0.000468814599)
( 0.0756463328, 0.000569265004)
( 0.0869749003, 0.000689820537)
( 0.1, 0.000833987797)
( 0.1149757, 0.00100570374)
( 0.132194115, 0.00120932638)
( 0.151991108, 0.00144960076)
( 0.17475284, 0.0017315936)
( 0.2009233, 0.00206059057)
( 0.23101297, 0.00244195128)
( 0.265608778, 0.00288091998)
( 0.305385551, 0.00338239302)
( 0.351119173, 0.00395064957)
( 0.403701726, 0.0045890571)
( 0.464158883, 0.00529976892)
( 0.533669923, 0.00608343573)
( 0.613590727, 0.00693895593)
( 0.705480231, 0.0078632897)
( 0.811130831, 0.00885135888)
( 0.932603347, 0.0098960486)
( 1.07226722, 0.0109883179)
( 1.23284674, 0.0121174165)
( 1.41747416, 0.0132711957)
( 1.62975083, 0.0144364917)
( 1.87381742, 0.0155995551)
( 2.15443469, 0.0167464978)
( 2.47707636, 0.0178637274)
( 2.84803587, 0.0189383464)
( 3.27454916, 0.0199584945)
( 3.76493581, 0.0209136229)
( 4.32876128, 0.0217946928)
( 4.97702356, 0.0225942988)
( 5.72236766, 0.0233067209)
( 6.57933225, 0.0239279135)
( 7.56463328, 0.0244554419)
( 8.69749003, 0.0248883762)
( 10, 0.0252271556)
( 11.49757, 0.0254734322)
( 13.2194115, 0.0256299039)
( 15.1991108, 0.0257001453)
( 17.475284, 0.0256884407)
( 20.09233, 0.0255996262)
( 23.101297, 0.025438943)
( 26.5608778, 0.0252119049)
( 30.5385551, 0.0249241801)
( 35.1119173, 0.024581489)
( 40.3701726, 0.024189517)
( 46.4158883, 0.0237538416)
( 53.3669923, 0.0232798737)
( 61.3590727, 0.0227728104)
( 70.5480231, 0.0222375995)
( 81.1130831, 0.0216789137)
( 93.2603347, 0.0211011326)
( 107.226722, 0.0205083331)
( 123.284674, 0.0199042848)
( 141.747416, 0.0192924512)
( 162.975083, 0.0186759943)
( 187.381742, 0.018057783)
( 215.443469, 0.0174404039)
( 247.707636, 0.0168261735)
( 284.803587, 0.0162171525)
( 327.454916, 0.0156151605)
( 376.493581, 0.0150217912)
( 432.876128, 0.0144384277)
( 497.702356, 0.0138662583)
( 572.236766, 0.0133062917)
( 657.933225, 0.0127593711)
( 756.463328, 0.0122261891)
( 869.749003, 0.0117073008)
( 1000, 0.011203137)
};
\addplot [thick,black]
coordinates {
( 0.001, 1.19300759e-5)
( 0.001149757, 1.43003187e-5)
( 0.00132194115, 1.71241227e-5)
( 0.00151991108, 2.04844737e-5)
( 0.0017475284, 2.4478715e-5)
( 0.002009233, 2.92208516e-5)
( 0.0023101297, 3.48441844e-5)
( 0.00265608778, 4.15043115e-5)
( 0.00305385551, 4.93825373e-5)
( 0.00351119173, 5.8689729e-5)
( 0.00403701726, 6.96706629e-5)
( 0.00464158883, 8.26089009e-5)
( 0.00533669923, 9.78322279e-5)
( 0.00613590727, 0.000115718699)
( 0.00705480231, 0.000136703302)
( 0.00811130831, 0.000161285253)
( 0.00932603347, 0.000190035932)
( 0.0107226722, 0.00022360742)
( 0.0123284674, 0.000262741592)
( 0.0141747416, 0.000308279669)
( 0.0162975083, 0.000361172113)
( 0.0187381742, 0.000422488666)
( 0.0215443469, 0.000493428283)
( 0.0247707636, 0.000575328663)
( 0.0284803587, 0.000669674942)
( 0.0327454916, 0.000778107094)
( 0.0376493581, 0.000902425416)
( 0.0432876128, 0.00104459343)
( 0.0497702356, 0.00120673743)
( 0.0572236766, 0.00139114175)
( 0.0657933225, 0.00160023885)
( 0.0756463328, 0.00183659325)
( 0.0869749003, 0.00210287824)
( 0.1, 0.00240184451)
( 0.1149757, 0.00273627984)
( 0.132194115, 0.00310895924)
( 0.151991108, 0.00352258517)
( 0.17475284, 0.00397971803)
( 0.2009233, 0.00448269738)
( 0.23101297, 0.00503355508)
( 0.265608778, 0.00563392228)
( 0.305385551, 0.0062849327)
( 0.351119173, 0.00698712555)
( 0.403701726, 0.00774035203)
( 0.464158883, 0.00854368976)
( 0.533669923, 0.00939537004)
( 0.613590727, 0.0102927227)
( 0.705480231, 0.0112321429)
( 0.811130831, 0.0122090843)
( 0.932603347, 0.0132180808)
( 1.07226722, 0.0142527983)
( 1.23284674, 0.0153061176)
( 1.41747416, 0.0163702446)
( 1.62975083, 0.0174368465)
( 1.87381742, 0.0184972069)
( 2.15443469, 0.0195423952)
( 2.47707636, 0.0205634426)
( 2.84803587, 0.0215515179)
( 3.27454916, 0.0224980962)
( 3.76493581, 0.0233951145)
( 4.32876128, 0.02423511)
( 4.97702356, 0.0250113358)
( 5.72236766, 0.0257178551)
( 6.57933225, 0.0263496094)
( 7.56463328, 0.026902464)
( 8.69749003, 0.0273732313)
( 10, 0.0277596728)
( 11.49757, 0.028060484)
( 13.2194115, 0.0282752639)
( 15.1991108, 0.0284044707)
( 17.475284, 0.0284493681)
( 20.09233, 0.0284119627)
( 23.101297, 0.0282949357)
( 26.5608778, 0.0281015693)
( 30.5385551, 0.0278356712)
( 35.1119173, 0.0275014964)
( 40.3701726, 0.0271036697)
( 46.4158883, 0.0266471086)
( 53.3669923, 0.0261369473)
( 61.3590727, 0.0255784649)
( 70.5480231, 0.0249770163)
( 81.1130831, 0.0243379669)
( 93.2603347, 0.0236666339)
( 107.226722, 0.0229682313)
( 123.284674, 0.0222478221)
( 141.747416, 0.0215102764)
( 162.975083, 0.020760235)
( 187.381742, 0.0200020807)
( 215.443469, 0.0192399147)
( 247.707636, 0.0184775395)
( 284.803587, 0.0177184476)
( 327.454916, 0.0169658151)
( 376.493581, 0.0162225004)
( 432.876128, 0.0154910471)
( 497.702356, 0.0147736907)
( 572.236766, 0.0140723684)
( 657.933225, 0.0133887317)
( 756.463328, 0.0127241611)
( 869.749003, 0.0120797824)
( 1000, 0.0114564841)
};
\addplot [thin,black]
coordinates {
( 0.001, 0.227224848)
( 0.001149757, 0.211866227)
( 0.00132194115, 0.197880327)
( 0.00151991108, 0.185137809)
( 0.0017475284, 0.17352193)
( 0.002009233, 0.162927297)
( 0.0023101297, 0.153258748)
( 0.00265608778, 0.144430338)
( 0.00305385551, 0.136364431)
( 0.00351119173, 0.128990879)
( 0.00403701726, 0.122246282)
( 0.00464158883, 0.116073325)
( 0.00533669923, 0.110420176)
( 0.00613590727, 0.105239948)
( 0.00705480231, 0.100490211)
( 0.00811130831, 0.0961325552)
( 0.00932603347, 0.0921321956)
( 0.0107226722, 0.0884576158)
( 0.0123284674, 0.0850802483)
( 0.0141747416, 0.0819741854)
( 0.0162975083, 0.0791159195)
( 0.0187381742, 0.0764841085)
( 0.0215443469, 0.0740593644)
( 0.0247707636, 0.0718240629)
( 0.0284803587, 0.0697621719)
( 0.0327454916, 0.0678590961)
( 0.0376493581, 0.0661015378)
( 0.0432876128, 0.0644773702)
( 0.0497702356, 0.0629755236)
( 0.0572236766, 0.0615858824)
( 0.0657933225, 0.0602991916)
( 0.0756463328, 0.0591069724)
( 0.0869749003, 0.0580014456)
( 0.1, 0.0569754616)
( 0.1149757, 0.0560224374)
( 0.132194115, 0.0551362986)
( 0.151991108, 0.0543114263)
( 0.17475284, 0.0535426089)
( 0.2009233, 0.0528249976)
( 0.23101297, 0.0521540652)
( 0.265608778, 0.0515255681)
( 0.305385551, 0.0509355117)
( 0.351119173, 0.0503801178)
( 0.403701726, 0.0498557947)
( 0.464158883, 0.049359109)
( 0.533669923, 0.0488867609)
( 0.613590727, 0.0484355606)
( 0.705480231, 0.0480024072)
( 0.811130831, 0.0475842703)
( 0.932603347, 0.0471781745)
( 1.07226722, 0.0467811857)
( 1.23284674, 0.0463904014)
( 1.41747416, 0.0460029443)
( 1.62975083, 0.045615959)
( 1.87381742, 0.0452266134)
( 2.15443469, 0.0448321035)
( 2.47707636, 0.0444296631)
( 2.84803587, 0.0440165772)
( 3.27454916, 0.0435902002)
( 3.76493581, 0.0431479774)
( 4.32876128, 0.0426874705)
( 4.97702356, 0.0422063856)
( 5.72236766, 0.0417026031)
( 6.57933225, 0.0411742097)
( 7.56463328, 0.0406195291)
( 8.69749003, 0.0400371527)
( 10, 0.0394259685)
( 11.49757, 0.0387851821)
( 13.2194115, 0.0381143443)
( 15.1991108, 0.0374133585)
( 17.475284, 0.0366824935)
( 20.09233, 0.0359223845)
( 23.101297, 0.035134028)
( 26.5608778, 0.0343187702)
( 30.5385551, 0.0334782877)
( 35.1119173, 0.0326145624)
( 40.3701726, 0.0317298509)
( 46.4158883, 0.0308266488)
( 53.3669923, 0.0299076512)
( 61.3590727, 0.0289756698)
( 70.5480231, 0.0280337956)
( 81.1130831, 0.0270849422)
( 93.2603347, 0.026132216)
( 107.226722, 0.0251786679)
( 123.284674, 0.0242272961)
( 141.747416, 0.0232810107)
( 162.975083, 0.0223426015)
( 187.381742, 0.0214147112)
( 215.443469, 0.0204998122)
( 247.707636, 0.0196001883)
( 284.803587, 0.0187179208)
( 327.454916, 0.0178548789)
( 376.493581, 0.0170127149)
( 432.876128, 0.0161928619)
( 497.702356, 0.0153965363)
( 572.236766, 0.0146247422)
( 657.933225, 0.0138782789)
( 756.463328, 0.0131577503)
( 869.749003, 0.0124635762)
( 1000, 0.0117960045)
};
\end{loglogaxis}


==> chivE1.tex <==
\begin{loglogaxis}[
xmin= 0.001, xmax= 0.1,
xlabel={$E/mc^2$},
ylabel={$\chi$},
ylabel near ticks,
]
\addplot []
coordinates {
( 0.001, 0.24620815)
( 0.00104761575, 0.240307298)
( 0.00109749877, 0.234553056)
( 0.001149757, 0.228941554)
( 0.00120450354, 0.223469035)
( 0.00126185688, 0.21813185)
( 0.00132194115, 0.212926453)
( 0.00138488637, 0.207849402)
( 0.00145082878, 0.20289735)
( 0.00151991108, 0.198067047)
( 0.00159228279, 0.193355334)
( 0.00166810054, 0.188759142)
( 0.0017475284, 0.184275486)
( 0.00183073828, 0.179901467)
( 0.00191791026, 0.175634266)
( 0.002009233, 0.171471142)
( 0.00210490414, 0.167409431)
( 0.00220513074, 0.16344654)
( 0.0023101297, 0.159579951)
( 0.00242012826, 0.155807213)
( 0.00253536449, 0.152125943)
( 0.00265608778, 0.148533823)
( 0.0027825594, 0.145028596)
( 0.00291505306, 0.14160807)
( 0.00305385551, 0.13827011)
( 0.00319926714, 0.135012638)
( 0.00335160265, 0.131833634)
( 0.00351119173, 0.128731131)
( 0.00367837977, 0.125703214)
( 0.00385352859, 0.122748021)
( 0.00403701726, 0.119863738)
( 0.00422924287, 0.117048599)
( 0.00443062146, 0.114300886)
( 0.00464158883, 0.111618925)
( 0.00486260158, 0.109001088)
( 0.00509413801, 0.106445788)
( 0.00533669923, 0.10395148)
( 0.00559081018, 0.101516659)
( 0.00585702082, 0.0991398615)
( 0.00613590727, 0.0968196596)
( 0.00642807312, 0.0945546629)
( 0.00673415066, 0.0923435177)
( 0.00705480231, 0.090184905)
( 0.00739072203, 0.0880775397)
( 0.00774263683, 0.0860201701)
( 0.00811130831, 0.0840115762)
( 0.00849753436, 0.0820505695)
( 0.00890215085, 0.0801359918)
( 0.00932603347, 0.0782667145)
( 0.00977009957, 0.0764416377)
( 0.0102353102, 0.0746596896)
( 0.0107226722, 0.0729198252)
( 0.0112332403, 0.0712210263)
( 0.0117681195, 0.0695623003)
( 0.0123284674, 0.0679426796)
( 0.0129154967, 0.066361221)
( 0.0135304777, 0.0648170051)
( 0.0141747416, 0.0633091352)
( 0.0148496826, 0.0618367375)
( 0.0155567614, 0.0603989597)
( 0.0162975083, 0.0589949709)
( 0.0170735265, 0.0576239609)
( 0.0178864953, 0.0562851396)
( 0.0187381742, 0.0549777365)
( 0.0196304065, 0.0537010004)
( 0.0205651231, 0.0524541984)
( 0.0215443469, 0.0512366158)
( 0.0225701972, 0.0500475557)
( 0.0236448941, 0.0488863383)
( 0.0247707636, 0.0477523003)
( 0.0259502421, 0.0466447949)
( 0.0271858824, 0.0455631913)
( 0.0284803587, 0.0445068738)
( 0.0298364724, 0.0434752421)
( 0.0312571585, 0.0424677104)
( 0.0327454916, 0.0414837072)
( 0.0343046929, 0.040522675)
( 0.0359381366, 0.0395840698)
( 0.0376493581, 0.0386673609)
( 0.0394420606, 0.0377720305)
( 0.041320124, 0.0368975732)
( 0.0432876128, 0.0360434961)
( 0.0453487851, 0.0352093179)
( 0.0475081016, 0.0343945693)
( 0.0497702356, 0.0335987921)
( 0.0521400829, 0.0328215392)
( 0.0546227722, 0.0320623743)
( 0.0572236766, 0.0313208717)
( 0.059948425, 0.0305966157)
( 0.0628029144, 0.0298892008)
( 0.0657933225, 0.0291982311)
( 0.068926121, 0.0285233204)
( 0.0722080902, 0.0278640914)
( 0.0756463328, 0.0272201763)
( 0.0792482898, 0.0265912156)
( 0.0830217568, 0.0259768588)
( 0.0869749003, 0.0253767636)
( 0.0911162756, 0.0247905958)
( 0.0954548457, 0.0242180292)
( 0.1, 0.0236587456)
};
\addplot []
coordinates {
( 0.001, 0.222419608)
( 0.00104761575, 0.217570654)
( 0.00109749877, 0.212822265)
( 0.001149757, 0.208172563)
( 0.00120450354, 0.203619693)
( 0.00126185688, 0.199161829)
( 0.00132194115, 0.194797172)
( 0.00138488637, 0.19052395)
( 0.00145082878, 0.186340418)
( 0.00151991108, 0.182244858)
( 0.00159228279, 0.178235576)
( 0.00166810054, 0.174310908)
( 0.0017475284, 0.170469213)
( 0.00183073828, 0.166708877)
( 0.00191791026, 0.163028314)
( 0.002009233, 0.15942596)
( 0.00210490414, 0.155900279)
( 0.00220513074, 0.152449759)
( 0.0023101297, 0.149072913)
( 0.00242012826, 0.14576828)
( 0.00253536449, 0.142534422)
( 0.00265608778, 0.139369925)
( 0.0027825594, 0.136273402)
( 0.00291505306, 0.133243486)
( 0.00305385551, 0.130278837)
( 0.00319926714, 0.127378135)
( 0.00335160265, 0.124540085)
( 0.00351119173, 0.121763415)
( 0.00367837977, 0.119046875)
( 0.00385352859, 0.116389238)
( 0.00403701726, 0.113789297)
( 0.00422924287, 0.111245869)
( 0.00443062146, 0.108757791)
( 0.00464158883, 0.106323922)
( 0.00486260158, 0.103943141)
( 0.00509413801, 0.10161435)
( 0.00533669923, 0.0993364674)
( 0.00559081018, 0.0971084354)
( 0.00585702082, 0.0949292141)
( 0.00613590727, 0.0927977835)
( 0.00642807312, 0.090713143)
( 0.00673415066, 0.0886743108)
( 0.00705480231, 0.0866803239)
( 0.00739072203, 0.0847302376)
( 0.00774263683, 0.0828231255)
( 0.00811130831, 0.0809580792)
( 0.00849753436, 0.0791342071)
( 0.00890215085, 0.077350636)
( 0.00932603347, 0.0756065092)
( 0.00977009957, 0.0739009866)
( 0.0102353102, 0.072233245)
( 0.0107226722, 0.0706024773)
( 0.0112332403, 0.0690078922)
( 0.0117681195, 0.0674487144)
( 0.0123284674, 0.0659241838)
( 0.0129154967, 0.0644335557)
( 0.0135304777, 0.0629761002)
( 0.0141747416, 0.0615511022)
( 0.0148496826, 0.0601578609)
( 0.0155567614, 0.0587956897)
( 0.0162975083, 0.0574639161)
( 0.0170735265, 0.0561618811)
( 0.0178864953, 0.0548889392)
( 0.0187381742, 0.0536444582)
( 0.0196304065, 0.0524278188)
( 0.0205651231, 0.0512384144)
( 0.0215443469, 0.050075651)
( 0.0225701972, 0.0489389468)
( 0.0236448941, 0.0478277321)
( 0.0247707636, 0.0467414491)
( 0.0259502421, 0.0456795515)
( 0.0271858824, 0.0446415044)
( 0.0284803587, 0.0436267842)
( 0.0298364724, 0.0426348782)
( 0.0312571585, 0.0416652844)
( 0.0327454916, 0.0407175116)
( 0.0343046929, 0.0397910786)
( 0.0359381366, 0.0388855148)
( 0.0376493581, 0.0380003591)
( 0.0394420606, 0.0371351606)
( 0.041320124, 0.0362894776)
( 0.0432876128, 0.0354628782)
( 0.0453487851, 0.0346549393)
( 0.0475081016, 0.0338652472)
( 0.0497702356, 0.0330933968)
( 0.0521400829, 0.0323389919)
( 0.0546227722, 0.0316016445)
( 0.0572236766, 0.0308809751)
( 0.059948425, 0.0301766126)
( 0.0628029144, 0.0294881935)
( 0.0657933225, 0.0288153624)
( 0.068926121, 0.0281577716)
( 0.0722080902, 0.0275150807)
( 0.0756463328, 0.026886957)
( 0.0792482898, 0.0262730747)
( 0.0830217568, 0.0256731153)
( 0.0869749003, 0.0250867671)
( 0.0911162756, 0.0245137255)
( 0.0954548457, 0.0239536921)
( 0.1, 0.0234063752)
};
\addplot []
coordinates {
( 0.001, 0.11000011)
( 0.00104761575, 0.108825028)
( 0.00109749877, 0.107647482)
( 0.001149757, 0.106467777)
( 0.00120450354, 0.105286223)
( 0.00126185688, 0.10410314)
( 0.00132194115, 0.102918849)
( 0.00138488637, 0.101733676)
( 0.00145082878, 0.100547953)
( 0.00151991108, 0.0993620123)
( 0.00159228279, 0.0981761905)
( 0.00166810054, 0.0969908248)
( 0.0017475284, 0.095806254)
( 0.00183073828, 0.0946228175)
( 0.00191791026, 0.0934408543)
( 0.002009233, 0.092260703)
( 0.00210490414, 0.091082701)
( 0.00220513074, 0.0899071838)
( 0.0023101297, 0.0887344846)
( 0.00242012826, 0.087564934)
( 0.00253536449, 0.086398859)
( 0.00265608778, 0.0852365831)
( 0.0027825594, 0.0840784254)
( 0.00291505306, 0.0829247003)
( 0.00305385551, 0.0817757175)
( 0.00319926714, 0.0806317808)
( 0.00335160265, 0.0794931884)
( 0.00351119173, 0.0783602324)
( 0.00367837977, 0.0772331983)
( 0.00385352859, 0.0761123649)
( 0.00403701726, 0.0749980039)
( 0.00422924287, 0.0738903798)
( 0.00443062146, 0.0727897494)
( 0.00464158883, 0.0716963618)
( 0.00486260158, 0.0706104584)
( 0.00509413801, 0.0695322723)
( 0.00533669923, 0.0684620283)
( 0.00559081018, 0.0673999429)
( 0.00585702082, 0.0663462242)
( 0.00613590727, 0.0653010717)
( 0.00642807312, 0.0642646763)
( 0.00673415066, 0.0632372201)
( 0.00705480231, 0.0622188766)
( 0.00739072203, 0.0612098106)
( 0.00774263683, 0.0602101781)
( 0.00811130831, 0.0592201264)
( 0.00849753436, 0.0582397944)
( 0.00890215085, 0.0572693118)
( 0.00932603347, 0.0563088004)
( 0.00977009957, 0.055358373)
( 0.0102353102, 0.0544181343)
( 0.0107226722, 0.0534881805)
( 0.0112332403, 0.0525685997)
( 0.0117681195, 0.0516594719)
( 0.0123284674, 0.0507608692)
( 0.0129154967, 0.0498728557)
( 0.0135304777, 0.0489954879)
( 0.0141747416, 0.048128815)
( 0.0148496826, 0.0472728785)
( 0.0155567614, 0.0464277127)
( 0.0162975083, 0.0455933452)
( 0.0170735265, 0.0447697964)
( 0.0178864953, 0.0439570801)
( 0.0187381742, 0.0431552036)
( 0.0196304065, 0.0423641678)
( 0.0205651231, 0.0415839677)
( 0.0215443469, 0.0408145921)
( 0.0225701972, 0.040056024)
( 0.0236448941, 0.0393082412)
( 0.0247707636, 0.0385712156)
( 0.0259502421, 0.0378449144)
( 0.0271858824, 0.0371292994)
( 0.0284803587, 0.036424328)
( 0.0298364724, 0.0357299526)
( 0.0312571585, 0.0350461215)
( 0.0327454916, 0.0343727785)
( 0.0343046929, 0.0337098636)
( 0.0359381366, 0.0330573128)
( 0.0376493581, 0.0324150584)
( 0.0394420606, 0.0317830292)
( 0.041320124, 0.031161151)
( 0.0432876128, 0.0305493459)
( 0.0453487851, 0.0299475335)
( 0.0475081016, 0.0293556304)
( 0.0497702356, 0.0287735506)
( 0.0521400829, 0.0282012056)
( 0.0546227722, 0.0276385045)
( 0.0572236766, 0.0270853545)
( 0.059948425, 0.0265416605)
( 0.0628029144, 0.0260073256)
( 0.0657933225, 0.0254822515)
( 0.068926121, 0.0249663378)
( 0.0722080902, 0.024459483)
( 0.0756463328, 0.0239615842)
( 0.0792482898, 0.0234725373)
( 0.0830217568, 0.0229922371)
( 0.0869749003, 0.0225205776)
( 0.0911162756, 0.0220574517)
( 0.0954548457, 0.021602752)
( 0.1, 0.02115637)
};
\addplot []
coordinates {
( 0.001, 0.015708527)
( 0.00104761575, 0.0156858484)
( 0.00109749877, 0.0156632625)
( 0.001149757, 0.0156407489)
( 0.00120450354, 0.015618287)
( 0.00126185688, 0.0155958559)
( 0.00132194115, 0.0155734348)
( 0.00138488637, 0.0155510023)
( 0.00145082878, 0.0155285372)
( 0.00151991108, 0.0155060179)
( 0.00159228279, 0.0154834225)
( 0.00166810054, 0.0154607289)
( 0.0017475284, 0.015437915)
( 0.00183073828, 0.0154149581)
( 0.00191791026, 0.0153918356)
( 0.002009233, 0.0153685245)
( 0.00210490414, 0.0153450014)
( 0.00220513074, 0.0153212429)
( 0.0023101297, 0.0152972252)
( 0.00242012826, 0.0152729243)
( 0.00253536449, 0.0152483161)
( 0.00265608778, 0.0152233759)
( 0.0027825594, 0.015198079)
( 0.00291505306, 0.0151724006)
( 0.00305385551, 0.0151463154)
( 0.00319926714, 0.0151197981)
( 0.00335160265, 0.0150928231)
( 0.00351119173, 0.0150653646)
( 0.00367837977, 0.0150373967)
( 0.00385352859, 0.0150088935)
( 0.00403701726, 0.0149798285)
( 0.00422924287, 0.0149501757)
( 0.00443062146, 0.0149199085)
( 0.00464158883, 0.0148890006)
( 0.00486260158, 0.0148574254)
( 0.00509413801, 0.0148251566)
( 0.00533669923, 0.0147921675)
( 0.00559081018, 0.0147584319)
( 0.00585702082, 0.0147239235)
( 0.00613590727, 0.0146886161)
( 0.00642807312, 0.0146524836)
( 0.00673415066, 0.0146155003)
( 0.00705480231, 0.0145776407)
( 0.00739072203, 0.0145388794)
( 0.00774263683, 0.0144991916)
( 0.00811130831, 0.0144585526)
( 0.00849753436, 0.0144169383)
( 0.00890215085, 0.0143743251)
( 0.00932603347, 0.0143306898)
( 0.00977009957, 0.0142860097)
( 0.0102353102, 0.014240263)
( 0.0107226722, 0.0141934281)
( 0.0112332403, 0.0141454846)
( 0.0117681195, 0.0140964125)
( 0.0123284674, 0.0140461928)
( 0.0129154967, 0.0139948072)
( 0.0135304777, 0.0139422384)
( 0.0141747416, 0.0138884701)
( 0.0148496826, 0.0138334868)
( 0.0155567614, 0.0137772742)
( 0.0162975083, 0.0137198191)
( 0.0170735265, 0.0136611093)
( 0.0178864953, 0.0136011339)
( 0.0187381742, 0.0135398831)
( 0.0196304065, 0.0134773484)
( 0.0205651231, 0.0134135227)
( 0.0215443469, 0.0133483999)
( 0.0225701972, 0.0132819755)
( 0.0236448941, 0.0132142464)
( 0.0247707636, 0.0131452108)
( 0.0259502421, 0.0130748682)
( 0.0271858824, 0.0130032198)
( 0.0284803587, 0.0129302682)
( 0.0298364724, 0.0128560173)
( 0.0312571585, 0.0127804726)
( 0.0327454916, 0.0127036412)
( 0.0343046929, 0.0126255315)
( 0.0359381366, 0.0125461535)
( 0.0376493581, 0.0124655187)
( 0.0394420606, 0.0123836402)
( 0.041320124, 0.0123005322)
( 0.0432876128, 0.0122162108)
( 0.0453487851, 0.0121306933)
( 0.0475081016, 0.0120439985)
( 0.0497702356, 0.0119561466)
( 0.0521400829, 0.0118671593)
( 0.0546227722, 0.0117770593)
( 0.0572236766, 0.011685871)
( 0.059948425, 0.01159362)
( 0.0628029144, 0.0115003329)
( 0.0657933225, 0.0114060379)
( 0.068926121, 0.0113107639)
( 0.0722080902, 0.0112145413)
( 0.0756463328, 0.0111174015)
( 0.0792482898, 0.0110193766)
( 0.0830217568, 0.0109205002)
( 0.0869749003, 0.0108208063)
( 0.0911162756, 0.01072033)
( 0.0954548457, 0.0106191072)
( 0.1, 0.0105171745)
};
\addplot []
coordinates {
( 0.001, 0.247364122)
( 0.00104761575, 0.241414176)
( 0.00109749877, 0.23561279)
( 0.001149757, 0.229956024)
( 0.00120450354, 0.224440055)
( 0.00126185688, 0.219061167)
( 0.00132194115, 0.213815752)
( 0.00138488637, 0.208700306)
( 0.00145082878, 0.203711422)
( 0.00151991108, 0.198845792)
( 0.00159228279, 0.194100201)
( 0.00166810054, 0.189471525)
( 0.0017475284, 0.184956728)
( 0.00183073828, 0.180552857)
( 0.00191791026, 0.176257045)
( 0.002009233, 0.172066503)
( 0.00210490414, 0.167978521)
( 0.00220513074, 0.163990462)
( 0.0023101297, 0.160099763)
( 0.00242012826, 0.156303933)
( 0.00253536449, 0.152600547)
( 0.00265608778, 0.14898725)
( 0.0027825594, 0.145461748)
( 0.00291505306, 0.14202181)
( 0.00305385551, 0.138665269)
( 0.00319926714, 0.135390013)
( 0.00335160265, 0.132193989)
( 0.00351119173, 0.129075198)
( 0.00367837977, 0.126031698)
( 0.00385352859, 0.123061595)
( 0.00403701726, 0.120163049)
( 0.00422924287, 0.117334268)
( 0.00443062146, 0.114573507)
( 0.00464158883, 0.111879068)
( 0.00486260158, 0.109249298)
( 0.00509413801, 0.106682589)
( 0.00533669923, 0.104177373)
( 0.00559081018, 0.101732125)
( 0.00585702082, 0.0993453593)
( 0.00613590727, 0.09701563)
( 0.00642807312, 0.0947415281)
( 0.00673415066, 0.0925216818)
( 0.00705480231, 0.0903547549)
( 0.00739072203, 0.0882394458)
( 0.00774263683, 0.0861744868)
( 0.00811130831, 0.0841586429)
( 0.00849753436, 0.0821907109)
( 0.00890215085, 0.0802695188)
( 0.00932603347, 0.0783939245)
( 0.00977009957, 0.0765628152)
( 0.0102353102, 0.0747751067)
( 0.0107226722, 0.0730297424)
( 0.0112332403, 0.0713256927)
( 0.0117681195, 0.0696619541)
( 0.0123284674, 0.0680375486)
( 0.0129154967, 0.0664515232)
( 0.0135304777, 0.0649029486)
( 0.0141747416, 0.0633909193)
( 0.0148496826, 0.0619145526)
( 0.0155567614, 0.0604729878)
( 0.0162975083, 0.059065386)
( 0.0170735265, 0.0576909293)
( 0.0178864953, 0.0563488203)
( 0.0187381742, 0.0550382813)
( 0.0196304065, 0.0537585545)
( 0.0205651231, 0.0525089004)
( 0.0215443469, 0.0512885983)
( 0.0225701972, 0.0500969452)
( 0.0236448941, 0.0489332556)
( 0.0247707636, 0.0477968611)
( 0.0259502421, 0.0466871094)
( 0.0271858824, 0.0456033649)
( 0.0284803587, 0.0445450071)
( 0.0298364724, 0.0435114312)
( 0.0312571585, 0.042502047)
( 0.0327454916, 0.0415162789)
( 0.0343046929, 0.0405535655)
( 0.0359381366, 0.0396133589)
( 0.0376493581, 0.0386951248)
( 0.0394420606, 0.0377983419)
( 0.041320124, 0.0369225015)
( 0.0432876128, 0.0360671076)
( 0.0453487851, 0.0352316758)
( 0.0475081016, 0.034415734)
( 0.0497702356, 0.0336188211)
( 0.0521400829, 0.0328404875)
( 0.0546227722, 0.0320802942)
( 0.0572236766, 0.0313378132)
( 0.059948425, 0.0306126265)
( 0.0628029144, 0.0299043264)
( 0.0657933225, 0.0292125149)
( 0.068926121, 0.0285368036)
( 0.0722080902, 0.0278768136)
( 0.0756463328, 0.027232175)
( 0.0792482898, 0.0266025267)
( 0.0830217568, 0.0259875165)
( 0.0869749003, 0.0253868004)
( 0.0911162756, 0.0248000428)
( 0.0954548457, 0.0242269161)
( 0.1, 0.0236671005)
};
\draw (axis cs:  0.003, 0.018) node {$\eta=0.1$};
\draw (axis cs:  0.003, 0.067) node {$0.01$    };
\draw (axis cs:  0.0018, 0.14) node {$0.001$   };
\end{loglogaxis}


==> chivE2.tex <==
\begin{loglogaxis}[
xmin= 0.001, xmax= 0.1,
xlabel={$E/mc^2$},
ylabel={$\chi$},
ylabel near ticks,
]
\addplot []
coordinates {
( 0.001, 0.189472682)
( 0.00104761575, 0.185853323)
( 0.00109749877, 0.182290319)
( 0.001149757, 0.178783296)
( 0.00120450354, 0.175331862)
( 0.00126185688, 0.171935605)
( 0.00132194115, 0.168594096)
( 0.00138488637, 0.165306887)
( 0.00145082878, 0.162073519)
( 0.00151991108, 0.158893514)
( 0.00159228279, 0.155766382)
( 0.00166810054, 0.152691621)
( 0.0017475284, 0.149668716)
( 0.00183073828, 0.146697144)
( 0.00191791026, 0.14377637)
( 0.002009233, 0.140905849)
( 0.00210490414, 0.138085031)
( 0.00220513074, 0.135313355)
( 0.0023101297, 0.132590257)
( 0.00242012826, 0.129915165)
( 0.00253536449, 0.127287502)
( 0.00265608778, 0.124706686)
( 0.0027825594, 0.122172133)
( 0.00291505306, 0.119683253)
( 0.00305385551, 0.117239456)
( 0.00319926714, 0.114840148)
( 0.00335160265, 0.112484733)
( 0.00351119173, 0.110172617)
( 0.00367837977, 0.107903203)
( 0.00385352859, 0.105675892)
( 0.00403701726, 0.10349009)
( 0.00422924287, 0.101345199)
( 0.00443062146, 0.0992406261)
( 0.00464158883, 0.0971757773)
( 0.00486260158, 0.0951500614)
( 0.00509413801, 0.0931628891)
( 0.00533669923, 0.091213674)
( 0.00559081018, 0.0893018322)
( 0.00585702082, 0.0874267831)
( 0.00613590727, 0.0855879494)
( 0.00642807312, 0.0837847574)
( 0.00673415066, 0.0820166373)
( 0.00705480231, 0.0802830235)
( 0.00739072203, 0.0785833545)
( 0.00774263683, 0.0769170736)
( 0.00811130831, 0.0752836286)
( 0.00849753436, 0.073682472)
( 0.00890215085, 0.0721130616)
( 0.00932603347, 0.0705748603)
( 0.00977009957, 0.0690673361)
( 0.0102353102, 0.0675899627)
( 0.0107226722, 0.066142219)
( 0.0112332403, 0.0647235898)
( 0.0117681195, 0.0633335654)
( 0.0123284674, 0.0619716422)
( 0.0129154967, 0.0606373221)
( 0.0135304777, 0.0593301132)
( 0.0141747416, 0.0580495296)
( 0.0148496826, 0.0567950913)
( 0.0155567614, 0.0555663245)
( 0.0162975083, 0.0543627615)
( 0.0170735265, 0.0531839408)
( 0.0178864953, 0.052029407)
( 0.0187381742, 0.050898711)
( 0.0196304065, 0.0497914098)
( 0.0205651231, 0.0487070668)
( 0.0215443469, 0.0476452513)
( 0.0225701972, 0.0466055392)
( 0.0236448941, 0.0455875123)
( 0.0247707636, 0.0445907587)
( 0.0259502421, 0.0436148728)
( 0.0271858824, 0.0426594548)
( 0.0284803587, 0.0417241115)
( 0.0298364724, 0.0408084553)
( 0.0312571585, 0.0399121052)
( 0.0327454916, 0.0390346857)
( 0.0343046929, 0.0381758278)
( 0.0359381366, 0.037335168)
( 0.0376493581, 0.0365123489)
( 0.0394420606, 0.0357070192)
( 0.041320124, 0.034918833)
( 0.0432876128, 0.0341474505)
( 0.0453487851, 0.0333925375)
( 0.0475081016, 0.0326537653)
( 0.0497702356, 0.0319308111)
( 0.0521400829, 0.0312233576)
( 0.0546227722, 0.0305310927)
( 0.0572236766, 0.0298537102)
( 0.059948425, 0.0291909089)
( 0.0628029144, 0.0285423931)
( 0.0657933225, 0.0279078723)
( 0.068926121, 0.0272870613)
( 0.0722080902, 0.0266796799)
( 0.0756463328, 0.0260854531)
( 0.0792482898, 0.0255041106)
( 0.0830217568, 0.0249353875)
( 0.0869749003, 0.0243790235)
( 0.0911162756, 0.023834763)
( 0.0954548457, 0.0233023555)
( 0.1, 0.0227815548)
};
\addplot []
coordinates {
( 0.001, 0.169165521)
( 0.00104761575, 0.166371913)
( 0.00109749877, 0.163603103)
( 0.001149757, 0.160859795)
( 0.00120450354, 0.158142647)
( 0.00126185688, 0.155452268)
( 0.00132194115, 0.152789221)
( 0.00138488637, 0.150154025)
( 0.00145082878, 0.147547155)
( 0.00151991108, 0.144969047)
( 0.00159228279, 0.142420092)
( 0.00166810054, 0.139900646)
( 0.0017475284, 0.137411025)
( 0.00183073828, 0.134951511)
( 0.00191791026, 0.132522348)
( 0.002009233, 0.13012375)
( 0.00210490414, 0.127755896)
( 0.00220513074, 0.125418935)
( 0.0023101297, 0.123112987)
( 0.00242012826, 0.120838143)
( 0.00253536449, 0.118594467)
( 0.00265608778, 0.116381997)
( 0.0027825594, 0.114200745)
( 0.00291505306, 0.112050702)
( 0.00305385551, 0.109931834)
( 0.00319926714, 0.107844087)
( 0.00335160265, 0.105787385)
( 0.00351119173, 0.103761634)
( 0.00367837977, 0.101766722)
( 0.00385352859, 0.0998025188)
( 0.00403701726, 0.0978688772)
( 0.00422924287, 0.0959656347)
( 0.00443062146, 0.0940926152)
( 0.00464158883, 0.0922496279)
( 0.00486260158, 0.0904364694)
( 0.00509413801, 0.0886529239)
( 0.00533669923, 0.0868987644)
( 0.00559081018, 0.0851737531)
( 0.00585702082, 0.0834776424)
( 0.00613590727, 0.0818101757)
( 0.00642807312, 0.0801710874)
( 0.00673415066, 0.0785601044)
( 0.00705480231, 0.0769769462)
( 0.00739072203, 0.0754213256)
( 0.00774263683, 0.0738929494)
( 0.00811130831, 0.0723915186)
( 0.00849753436, 0.0709167295)
( 0.00890215085, 0.0694682736)
( 0.00932603347, 0.0680458385)
( 0.00977009957, 0.0666491084)
( 0.0102353102, 0.0652777639)
( 0.0107226722, 0.0639314834)
( 0.0112332403, 0.0626099426)
( 0.0117681195, 0.0613128155)
( 0.0123284674, 0.0600397744)
( 0.0129154967, 0.0587904906)
( 0.0135304777, 0.0575646342)
( 0.0141747416, 0.056361875)
( 0.0148496826, 0.0551818824)
( 0.0155567614, 0.0540243259)
( 0.0162975083, 0.0528888751)
( 0.0170735265, 0.0517752004)
( 0.0178864953, 0.0506829727)
( 0.0187381742, 0.0496118642)
( 0.0196304065, 0.048561548)
( 0.0205651231, 0.0475316988)
( 0.0215443469, 0.0465219929)
( 0.0225701972, 0.0455321082)
( 0.0236448941, 0.0445617249)
( 0.0247707636, 0.0436105249)
( 0.0259502421, 0.0426781925)
( 0.0271858824, 0.0417644146)
( 0.0284803587, 0.0408688802)
( 0.0298364724, 0.0399912813)
( 0.0312571585, 0.0391313124)
( 0.0327454916, 0.0382886708)
( 0.0343046929, 0.037463057)
( 0.0359381366, 0.0366541742)
( 0.0376493581, 0.0358617289)
( 0.0394420606, 0.0350854306)
( 0.041320124, 0.0343249922)
( 0.0432876128, 0.0335801296)
( 0.0453487851, 0.0328505623)
( 0.0475081016, 0.0321360131)
( 0.0497702356, 0.0314362081)
( 0.0521400829, 0.030750877)
( 0.0546227722, 0.0300797528)
( 0.0572236766, 0.0294225723)
( 0.059948425, 0.0287790755)
( 0.0628029144, 0.0281490062)
( 0.0657933225, 0.0275321115)
( 0.068926121, 0.0269281424)
( 0.0722080902, 0.0263368531)
( 0.0756463328, 0.0257580016)
( 0.0792482898, 0.0251913495)
( 0.0830217568, 0.0246366619)
( 0.0869749003, 0.0240937073)
( 0.0911162756, 0.0235622581)
( 0.0954548457, 0.0230420899)
( 0.1, 0.022532982)
};
\addplot []
coordinates {
( 0.001, 0.0758795411)
( 0.00104761575, 0.0757247009)
( 0.00109749877, 0.0755438726)
( 0.001149757, 0.0753375643)
( 0.00120450354, 0.0751063069)
( 0.00126185688, 0.0748506513)
( 0.00132194115, 0.0745711676)
( 0.00138488637, 0.0742684433)
( 0.00145082878, 0.0739430815)
( 0.00151991108, 0.0735956997)
( 0.00159228279, 0.0732269282)
( 0.00166810054, 0.0728374086)
( 0.0017475284, 0.072427792)
( 0.00183073828, 0.0719987384)
( 0.00191791026, 0.0715509143)
( 0.002009233, 0.071084992)
( 0.00210490414, 0.0706016482)
( 0.00220513074, 0.0701015625)
( 0.0023101297, 0.0695854165)
( 0.00242012826, 0.0690538922)
( 0.00253536449, 0.0685076711)
( 0.00265608778, 0.0679474334)
( 0.0027825594, 0.0673738562)
( 0.00291505306, 0.0667876132)
( 0.00305385551, 0.0661893736)
( 0.00319926714, 0.0655798008)
( 0.00335160265, 0.0649595521)
( 0.00351119173, 0.0643292776)
( 0.00367837977, 0.0636896193)
( 0.00385352859, 0.0630412109)
( 0.00403701726, 0.0623846766)
( 0.00422924287, 0.0617206308)
( 0.00443062146, 0.0610496775)
( 0.00464158883, 0.0603724095)
( 0.00486260158, 0.0596894086)
( 0.00509413801, 0.0590012442)
( 0.00533669923, 0.0583084739)
( 0.00559081018, 0.0576116423)
( 0.00585702082, 0.0569112813)
( 0.00613590727, 0.0562079096)
( 0.00642807312, 0.0555020324)
( 0.00673415066, 0.0547941412)
( 0.00705480231, 0.0540847138)
( 0.00739072203, 0.0533742141)
( 0.00774263683, 0.0526630918)
( 0.00811130831, 0.0519517827)
( 0.00849753436, 0.0512407084)
( 0.00890215085, 0.0505302763)
( 0.00932603347, 0.0498208796)
( 0.00977009957, 0.0491128976)
( 0.0102353102, 0.0484066952)
( 0.0107226722, 0.0477026238)
( 0.0112332403, 0.0470010206)
( 0.0117681195, 0.0463022091)
( 0.0123284674, 0.0456064994)
( 0.0129154967, 0.0449141879)
( 0.0135304777, 0.044225558)
( 0.0141747416, 0.0435408798)
( 0.0148496826, 0.0428604105)
( 0.0155567614, 0.0421843949)
( 0.0162975083, 0.041513065)
( 0.0170735265, 0.0408466409)
( 0.0178864953, 0.0401853305)
( 0.0187381742, 0.0395293302)
( 0.0196304065, 0.0388788246)
( 0.0205651231, 0.0382339875)
( 0.0215443469, 0.0375949813)
( 0.0225701972, 0.0369619582)
( 0.0236448941, 0.0363350597)
( 0.0247707636, 0.0357144173)
( 0.0259502421, 0.0351001526)
( 0.0271858824, 0.0344923777)
( 0.0284803587, 0.0338911955)
( 0.0298364724, 0.0332966997)
( 0.0312571585, 0.0327089755)
( 0.0327454916, 0.0321280996)
( 0.0343046929, 0.0315541405)
( 0.0359381366, 0.0309871589)
( 0.0376493581, 0.030427208)
( 0.0394420606, 0.0298743334)
( 0.041320124, 0.029328574)
( 0.0432876128, 0.0287899616)
( 0.0453487851, 0.0282585217)
( 0.0475081016, 0.0277342735)
( 0.0497702356, 0.0272172301)
( 0.0521400829, 0.026707399)
( 0.0546227722, 0.0262047821)
( 0.0572236766, 0.0257093759)
( 0.059948425, 0.0252211722)
( 0.0628029144, 0.0247401577)
( 0.0657933225, 0.0242663148)
( 0.068926121, 0.0237996212)
( 0.0722080902, 0.0233400507)
( 0.0756463328, 0.0228875733)
( 0.0792482898, 0.022442155)
( 0.0830217568, 0.0220037584)
( 0.0869749003, 0.0215723429)
( 0.0911162756, 0.0211478644)
( 0.0954548457, 0.0207302763)
( 0.1, 0.0203195289)
};
\addplot []
coordinates {
( 0.001, 0.00577318671)
( 0.00104761575, 0.00590584753)
( 0.00109749877, 0.00603894979)
( 0.001149757, 0.00617239167)
( 0.00120450354, 0.0063060699)
( 0.00126185688, 0.00643988002)
( 0.00132194115, 0.00657371657)
( 0.00138488637, 0.0067074733)
( 0.00145082878, 0.00684104343)
( 0.00151991108, 0.00697431987)
( 0.00159228279, 0.00710719543)
( 0.00166810054, 0.00723956304)
( 0.0017475284, 0.00737131597)
( 0.00183073828, 0.00750234806)
( 0.00191791026, 0.00763255391)
( 0.002009233, 0.00776182906)
( 0.00210490414, 0.00789007025)
( 0.00220513074, 0.00801717554)
( 0.0023101297, 0.00814304449)
( 0.00242012826, 0.0082675784)
( 0.00253536449, 0.00839068038)
( 0.00265608778, 0.00851225555)
( 0.0027825594, 0.00863221115)
( 0.00291505306, 0.00875045671)
( 0.00305385551, 0.00886690412)
( 0.00319926714, 0.00898146778)
( 0.00335160265, 0.00909406464)
( 0.00351119173, 0.00920461435)
( 0.00367837977, 0.00931303929)
( 0.00385352859, 0.00941926466)
( 0.00403701726, 0.00952321851)
( 0.00422924287, 0.00962483183)
( 0.00443062146, 0.00972403853)
( 0.00464158883, 0.00982077552)
( 0.00486260158, 0.00991498268)
( 0.00509413801, 0.0100066029)
( 0.00533669923, 0.0100955821)
( 0.00559081018, 0.0101818693)
( 0.00585702082, 0.0102654163)
( 0.00613590727, 0.0103461781)
( 0.00642807312, 0.0104241125)
( 0.00673415066, 0.0104991804)
( 0.00705480231, 0.0105713456)
( 0.00739072203, 0.0106405746)
( 0.00774263683, 0.010706837)
( 0.00811130831, 0.0107701051)
( 0.00849753436, 0.010830354)
( 0.00890215085, 0.0108875614)
( 0.00932603347, 0.0109417079)
( 0.00977009957, 0.0109927766)
( 0.0102353102, 0.0110407533)
( 0.0107226722, 0.0110856263)
( 0.0112332403, 0.0111273864)
( 0.0117681195, 0.0111660269)
( 0.0123284674, 0.0112015435)
( 0.0129154967, 0.0112339343)
( 0.0135304777, 0.0112631997)
( 0.0141747416, 0.0112893423)
( 0.0148496826, 0.0113123672)
( 0.0155567614, 0.0113322814)
( 0.0162975083, 0.0113490943)
( 0.0170735265, 0.0113628171)
( 0.0178864953, 0.0113734635)
( 0.0187381742, 0.0113810489)
( 0.0196304065, 0.0113855907)
( 0.0205651231, 0.0113871085)
( 0.0215443469, 0.0113856236)
( 0.0225701972, 0.0113811592)
( 0.0236448941, 0.0113737403)
( 0.0247707636, 0.011363394)
( 0.0259502421, 0.0113501486)
( 0.0271858824, 0.0113340347)
( 0.0284803587, 0.0113150841)
( 0.0298364724, 0.0112933305)
( 0.0312571585, 0.0112688093)
( 0.0327454916, 0.0112415571)
( 0.0343046929, 0.0112116123)
( 0.0359381366, 0.0111790146)
( 0.0376493581, 0.0111438054)
( 0.0394420606, 0.0111060272)
( 0.041320124, 0.011065724)
( 0.0432876128, 0.011022941)
( 0.0453487851, 0.0109777247)
( 0.0475081016, 0.0109301228)
( 0.0497702356, 0.0108801841)
( 0.0521400829, 0.0108279587)
( 0.0546227722, 0.0107734974)
( 0.0572236766, 0.0107168523)
( 0.059948425, 0.0106580764)
( 0.0628029144, 0.0105972233)
( 0.0657933225, 0.0105343479)
( 0.068926121, 0.0104695054)
( 0.0722080902, 0.0104027521)
( 0.0756463328, 0.0103341448)
( 0.0792482898, 0.0102637408)
( 0.0830217568, 0.010191598)
( 0.0869749003, 0.0101177749)
( 0.0911162756, 0.0100423303)
( 0.0954548457, 0.0099653233)
( 0.1, 0.00988681344)
};
\addplot []
coordinates {
( 0.001, 0.201492729)
( 0.00104761575, 0.197528754)
( 0.00109749877, 0.193629253)
( 0.001149757, 0.189793732)
( 0.00120450354, 0.186021678)
( 0.00126185688, 0.182312556)
( 0.00132194115, 0.178665814)
( 0.00138488637, 0.175080883)
( 0.00145082878, 0.171557176)
( 0.00151991108, 0.168094096)
( 0.00159228279, 0.164691026)
( 0.00166810054, 0.161347341)
( 0.0017475284, 0.158062402)
( 0.00183073828, 0.154835561)
( 0.00191791026, 0.151666158)
( 0.002009233, 0.148553527)
( 0.00210490414, 0.145496991)
( 0.00220513074, 0.14249587)
( 0.0023101297, 0.139549473)
( 0.00242012826, 0.136657107)
( 0.00253536449, 0.133818075)
( 0.00265608778, 0.131031672)
( 0.0027825594, 0.128297195)
( 0.00291505306, 0.125613934)
( 0.00305385551, 0.122981181)
( 0.00319926714, 0.120398225)
( 0.00335160265, 0.117864353)
( 0.00351119173, 0.115378855)
( 0.00367837977, 0.112941019)
( 0.00385352859, 0.110550136)
( 0.00403701726, 0.108205497)
( 0.00422924287, 0.105906396)
( 0.00443062146, 0.10365213)
( 0.00464158883, 0.101441997)
( 0.00486260158, 0.0992753001)
( 0.00509413801, 0.0971513447)
( 0.00533669923, 0.0950694411)
( 0.00559081018, 0.0930289039)
( 0.00585702082, 0.0910290519)
( 0.00613590727, 0.0890692094)
( 0.00642807312, 0.0871487055)
( 0.00673415066, 0.085266875)
( 0.00705480231, 0.0834230584)
( 0.00739072203, 0.0816166023)
( 0.00774263683, 0.0798468591)
( 0.00811130831, 0.0781131879)
( 0.00849753436, 0.0764149541)
( 0.00890215085, 0.0747515299)
( 0.00932603347, 0.0731222944)
( 0.00977009957, 0.0715266335)
( 0.0102353102, 0.0699639402)
( 0.0107226722, 0.0684336148)
( 0.0112332403, 0.0669350649)
( 0.0117681195, 0.0654677052)
( 0.0123284674, 0.0640309583)
( 0.0129154967, 0.0626242538)
( 0.0135304777, 0.0612470294)
( 0.0141747416, 0.0598987299)
( 0.0148496826, 0.0585788081)
( 0.0155567614, 0.0572867242)
( 0.0162975083, 0.0560219465)
( 0.0170735265, 0.0547839505)
( 0.0178864953, 0.0535722197)
( 0.0187381742, 0.0523862453)
( 0.0196304065, 0.0512255262)
( 0.0205651231, 0.0500895687)
( 0.0215443469, 0.0489778872)
( 0.0225701972, 0.0478900034)
( 0.0236448941, 0.0468254468)
( 0.0247707636, 0.0457837543)
( 0.0259502421, 0.0447644705)
( 0.0271858824, 0.0437671473)
( 0.0284803587, 0.0427913441)
( 0.0298364724, 0.0418366278)
( 0.0312571585, 0.0409025724)
( 0.0327454916, 0.0399887594)
( 0.0343046929, 0.0390947774)
( 0.0359381366, 0.038220222)
( 0.0376493581, 0.0373646961)
( 0.0394420606, 0.0365278095)
( 0.041320124, 0.0357091789)
( 0.0432876128, 0.0349084278)
( 0.0453487851, 0.0341251867)
( 0.0475081016, 0.0333590926)
( 0.0497702356, 0.0326097892)
( 0.0521400829, 0.0318769268)
( 0.0546227722, 0.031160162)
( 0.0572236766, 0.0304591579)
( 0.059948425, 0.0297735839)
( 0.0628029144, 0.0291031157)
( 0.0657933225, 0.028447435)
( 0.068926121, 0.0278062295)
( 0.0722080902, 0.0271791931)
( 0.0756463328, 0.0265660253)
( 0.0792482898, 0.0259664315)
( 0.0830217568, 0.025380123)
( 0.0869749003, 0.0248068164)
( 0.0911162756, 0.0242462341)
( 0.0954548457, 0.0236981038)
( 0.1, 0.0231621586)
};
\draw (axis cs:  0.003, 0.011) node {$\eta=0.1$};
\draw (axis cs:  0.003, 0.055) node {$0.01$    };
\draw (axis cs:  0.0018, 0.11) node {$0.001$   };
\end{loglogaxis}


==> yfig.tex <==
\begin{loglogaxis}[
xmin= 0.0001, xmax= 100,
xlabel={$\Omega$},
ylabel={$y$},
ylabel near ticks,
grid=both
]
\addplot []
coordinates {
( 0.0001, 0.000723184604)
( 0.0001149757, 0.000817405409)
( 0.000132194115, 0.000923662006)
( 0.000151991108, 0.00104345246)
( 0.00017475284, 0.00117845473)
( 0.0002009233, 0.00133054724)
( 0.00023101297, 0.00150183156)
( 0.000265608778, 0.00169465702)
( 0.000305385551, 0.00191164911)
( 0.000351119173, 0.00215573891)
( 0.000403701726, 0.0024301968)
( 0.000464158883, 0.0027386689)
( 0.000533669923, 0.00308521701)
( 0.000613590727, 0.00347436202)
( 0.000705480231, 0.00391113193)
( 0.000811130831, 0.004401113)
( 0.000932603347, 0.00495050617)
( 0.00107226722, 0.00556618735)
( 0.00123284674, 0.00625577326)
( 0.00141747416, 0.00702769101)
( 0.00162975083, 0.00789125392)
( 0.00187381742, 0.0088567412)
( 0.00215443469, 0.00993548317)
( 0.00247707636, 0.011139951)
( 0.00284803587, 0.0124838509)
( 0.00327454916, 0.0139822221)
( 0.00376493581, 0.0156515386)
( 0.00432876128, 0.0175098127)
( 0.00497702356, 0.0195767)
( 0.00572236766, 0.0218736051)
( 0.00657933225, 0.0244237833)
( 0.00756463328, 0.0272524402)
( 0.00869749003, 0.0303868229)
( 0.01, 0.0338563014)
( 0.01149757, 0.0376924358)
( 0.0132194115, 0.0419290249)
( 0.0151991108, 0.0466021307)
( 0.017475284, 0.0517500729)
( 0.02009233, 0.0574133867)
( 0.023101297, 0.0636347357)
( 0.0265608778, 0.070458772)
( 0.0305385551, 0.0779319336)
( 0.0351119173, 0.0861021695)
( 0.0403701726, 0.0950185814)
( 0.0464158883, 0.104730972)
( 0.0533669923, 0.115289288)
( 0.0613590727, 0.126742949)
( 0.0705480231, 0.139140052)
( 0.0811130831, 0.152526444)
( 0.0932603347, 0.166944662)
( 0.107226722, 0.182432732)
( 0.123284674, 0.199022845)
( 0.141747416, 0.21673991)
( 0.162975083, 0.235600007)
( 0.187381742, 0.255608783)
( 0.215443469, 0.276759812)
( 0.247707636, 0.299032995)
( 0.284803587, 0.322393052)
( 0.327454916, 0.346788201)
( 0.376493581, 0.372149104)
( 0.432876128, 0.398388192)
( 0.497702356, 0.425399463)
( 0.572236766, 0.453058861)
( 0.657933225, 0.481225315)
( 0.756463328, 0.509742499)
( 0.869749003, 0.538441348)
( 1, 0.56714329)
( 1.149757, 0.595664141)
( 1.32194115, 0.6238185)
( 1.51991108, 0.651424479)
( 1.7475284, 0.678308509)
( 2.009233, 0.704309965)
( 2.3101297, 0.729285338)
( 2.65608778, 0.753111701)
( 3.05385551, 0.77568927)
( 3.51119173, 0.796942932)
( 4.03701726, 0.816822701)
( 4.64158883, 0.83530312)
( 5.33669923, 0.852381759)
( 6.13590727, 0.868076952)
( 7.05480231, 0.882425012)
( 8.11130831, 0.895477122)
( 9.32603347, 0.907296128)
( 10.7226722, 0.917953409)
( 12.3284674, 0.927525965)
( 14.1747416, 0.936093824)
( 16.2975083, 0.943737826)
( 18.7381742, 0.950537805)
( 21.5443469, 0.956571157)
( 24.7707636, 0.961911773)
( 28.4803587, 0.9666293)
( 32.7454916, 0.970788663)
( 37.6493581, 0.974449831)
( 43.2876128, 0.977667748)
( 49.7702356, 0.980492407)
( 57.2236766, 0.982969032)
( 65.7933225, 0.985138315)
( 75.6463328, 0.987036712)
( 86.9749003, 0.988696757)
( 100, 0.990147384)
};
\end{loglogaxis}


==> yoverfig.tex <==
\begin{loglogaxis}[
xmin= 0.0001, xmax= 100,
ymin= 0.01, ymax= 1,
xlabel={$\Omega$},
ylabel={$y/\sqrt{\Omega}$},
ylabel near ticks,
grid=both
]
\addplot []
coordinates {
( 0.0001, 0.0723184604)
( 0.0001149757, 0.076231502)
( 0.000132194115, 0.0803354109)
( 0.000151991108, 0.0846376457)
( 0.00017475284, 0.0891457788)
( 0.0002009233, 0.0938674774)
( 0.00023101297, 0.098810488)
( 0.000265608778, 0.103982584)
( 0.000305385551, 0.109391591)
( 0.000351119173, 0.115045302)
( 0.000403701726, 0.120951467)
( 0.000464158883, 0.12711775)
( 0.000533669923, 0.133551679)
( 0.000613590727, 0.140260595)
( 0.000705480231, 0.147251606)
( 0.000811130831, 0.154531516)
( 0.000932603347, 0.162106758)
( 0.00107226722, 0.169983319)
( 0.00123284674, 0.178166666)
( 0.00141747416, 0.186661642)
( 0.00162975083, 0.195472385)
( 0.00187381742, 0.204602209)
( 0.00215443469, 0.214053496)
( 0.00247707636, 0.223827572)
( 0.00284803587, 0.233924573)
( 0.00327454916, 0.244343303)
( 0.00376493581, 0.255081081)
( 0.00432876128, 0.266133583)
( 0.00497702356, 0.277494664)
( 0.00572236766, 0.289156187)
( 0.00657933225, 0.301107816)
( 0.00756463328, 0.313336838)
( 0.00869749003, 0.325827942)
( 0.01, 0.338563014)
( 0.01149757, 0.351520918)
( 0.0132194115, 0.364677276)
( 0.0151991108, 0.37800425)
( 0.017475284, 0.391470324)
( 0.02009233, 0.405040093)
( 0.023101297, 0.418674068)
( 0.0265608778, 0.432328491)
( 0.0305385551, 0.445955176)
( 0.0351119173, 0.459501382)
( 0.0403701726, 0.472909719)
( 0.0464158883, 0.486118109)
( 0.0533669923, 0.499059805)
( 0.0613590727, 0.511663472)
( 0.0705480231, 0.523853363)
( 0.0811130831, 0.53554959)
( 0.0932603347, 0.546668503)
( 0.107226722, 0.557123204)
( 0.123284674, 0.566824202)
( 0.141747416, 0.575680227)
( 0.162975083, 0.583599207)
( 0.187381742, 0.590489441)
( 0.215443469, 0.59626094)
( 0.247707636, 0.600826962)
( 0.284803587, 0.604105718)
( 0.327454916, 0.60602223)
( 0.376493581, 0.606510313)
( 0.432876128, 0.605514628)
( 0.497702356, 0.602992747)
( 0.572236766, 0.598917151)
( 0.657933225, 0.59327706)
( 0.756463328, 0.586080004)
( 0.869749003, 0.577353008)
( 1, 0.56714329)
( 1.149757, 0.555518372)
( 1.32194115, 0.542565518)
( 1.51991108, 0.528390479)
( 1.7475284, 0.513115511)
( 2.009233, 0.496876757)
( 2.3101297, 0.479821054)
( 2.65608778, 0.462102356)
( 3.05385551, 0.443877919)
( 3.51119173, 0.425304474)
( 4.03701726, 0.406534583)
( 4.64158883, 0.387713364)
( 5.33669923, 0.368975715)
( 6.13590727, 0.350444164)
( 7.05480231, 0.332227353)
( 8.11130831, 0.314419187)
( 9.32603347, 0.297098578)
( 10.7226722, 0.280329708)
( 12.3284674, 0.264162722)
( 14.1747416, 0.248634737)
( 16.2975083, 0.233771066)
( 18.7381742, 0.219586562)
( 21.5443469, 0.206087008)
( 24.7707636, 0.193270488)
( 28.4803587, 0.181128682)
( 32.7454916, 0.169648076)
( 37.6493581, 0.158811043)
( 43.2876128, 0.148596805)
( 49.7702356, 0.138982265)
( 57.2236766, 0.129942721)
( 65.7933225, 0.121452456)
( 75.6463328, 0.113485236)
( 86.9749003, 0.106014713)
( 100, 0.0990147384)
};
\end{loglogaxis}

